Sparse Forcing: Native Trainable Sparse Attention for Real-time Autoregressive Diffusion Video Generation

We introduce Sparse Forcing, a training-and-inference paradigm for autoregressive video diffusion models that improves long-horizon generation quality while reducing decoding latency. Sparse Forcing is motivated by an empirical observation in autoregressive diffusion rollouts: attention concentrates on a persistent subset of salient visual blocks, forming an implicit spatiotemporal memory in the KV cache, and exhibits a locally structured block-sparse pattern within sliding windows. Building on this observation, we propose a trainable native sparsity mechanism that learns to compress, preserve, and update these persistent blocks while restricting computation within each local window to a dynamically selected local neighborhood. To make the approach practical at scale for both training and inference, we further propose Persistent Block-Sparse Attention (PBSA), an efficient GPU kernel that accelerates sparse attention and memory updates for low-latency, memory-efficient decoding. Experiments show that Sparse Forcing improves the VBench score by +0.26 over Self-Forcing on 5-second text-to-video generation while delivering a 1.11-1.17x decoding speedup and 42% lower peak KV-cache footprint. The gains are more pronounced on longer-horizon rollouts, delivering improved visual quality with +0.68 and +2.74 VBench improvements, and 1.22x and 1.27x speedups on 20-second and 1-minute generations, respectively.

==> algorithms/self_forcing_inference.tex <==
\begin{algorithm}[t]
\caption{Autoregressive Diffusion Inference with Rolling KV Cache}
\begin{algorithmic}[1]
\REQUIRE KV cache of size $L$ frames
\REQUIRE Denoise timesteps $\{t_1, \ldots, t_T\}$
\REQUIRE Number of generated frames $M$
\REQUIRE AR diffusion model $G_{\theta}$ (returns KV embeddings via $G^{KV}_{\theta}$)
\STATE Initialize model output $X_{\theta} \leftarrow [\,]$
\STATE Initialize KV cache $KV \leftarrow [\,]$
\FOR{$i = 1, \ldots, M$}
  \STATE Initialize $x^{i}_{t_T} \sim \mathcal{N}(0, I)$
  \FOR{$j = T, \ldots, 1$}
    \STATE Set $\hat{x}^{i}_{0} \leftarrow G_{\theta}(x^{i}_{t_j}; t_j, KV)$
    \IF{$j = 1$}
      \STATE $X_{\theta}.\mathrm{append}(\hat{x}^{i}_{0})$
      \STATE Cache $kv_i \leftarrow G^{KV}_{\theta}(\hat{x}^{i}_{0}; 0, KV)$
      \IF{$|KV| = L$}
        \STATE $KV.\mathrm{pop}(0)$ \COMMENT{Cache eviction}
      \ENDIF
      \STATE $KV.\mathrm{append}(kv_i)$
    \ELSE
      \STATE Sample $\epsilon \sim \mathcal{N}(0, I)$
      \STATE Set $x^{i}_{t_{j-1}} \leftarrow \Psi(\hat{x}^{i}_{0}, \epsilon, t_{j-1})$
    \ENDIF
  \ENDFOR
\ENDFOR
\STATE \textbf{return} $X_{\theta}$
\end{algorithmic}
\end{algorithm}

==> algorithms/self_forcing_training.tex <==
\begin{algorithm}[t]
\caption{Self Forcing Training}
\begin{algorithmic}[1]
\REQUIRE Denoise timesteps $\{t_1, \ldots, t_T\}$
\REQUIRE Number of video frames $N$
\REQUIRE AR diffusion model $G_{\theta}$ (returns KV embeddings via $G^{KV}_{\theta}$)
\LOOP
  \STATE Initialize model output $X_{\theta} \leftarrow [\,]$
  \STATE Initialize KV cache $KV \leftarrow [\,]$
  \STATE Sample $s \sim \mathrm{Uniform}(1,2,\ldots,T)$
  \FOR{$i = 1, \ldots, N$}
    \STATE Initialize $x^{i}_{t_T} \sim \mathcal{N}(0, I)$
    \FOR{$j = T, \ldots, s$}
      \IF{$j = s$}
        \STATE Enable gradient computation
        \STATE Set $\hat{x}^{i}_{0} \leftarrow G_{\theta}(x^{i}_{t_j}; t_j, KV)$
        \STATE $X_{\theta}.\mathrm{append}(\hat{x}^{i}_{0})$
        \STATE Disable gradient computation
        \STATE Cache $kv_i \leftarrow G^{KV}_{\theta}(\hat{x}^{i}_{0}; 0, KV)$
        \STATE $KV.\mathrm{append}(kv_i)$
      \ELSE
        \STATE Disable gradient computation
        \STATE Set $\hat{x}^{i}_{0} \leftarrow G_{\theta}(x^{i}_{t_j}; t_j, KV)$
        \STATE Sample $\epsilon \sim \mathcal{N}(0, I)$
        \STATE Set $x^{i}_{t_{j-1}} \leftarrow \Psi(\hat{x}^{i}_{0}, \epsilon, t_{j-1})$
      \ENDIF
    \ENDFOR
  \ENDFOR
  \STATE Update $\theta$ via distribution matching loss
\ENDLOOP
\end{algorithmic}
\end{algorithm}


==> algorithms/sparse_forcing_inference_old.tex <==
% \begin{algorithm}[t]
% \caption{Autoregressive Diffusion Inference with Rolling KV Cache in Sparse Forcing}
% \begin{algorithmic}[1]
% \REQUIRE KV cache of size $L$ frames
% \REQUIRE Denoise timesteps $\{t_1, \ldots, t_T\}$
% \REQUIRE Number of generated frames $M$
% \REQUIRE AR diffusion model $G_{\theta}$ (returns KV embeddings via $G^{KV}_{\theta}$)
% \STATE Initialize model output $X_{\theta} \leftarrow [\,]$
% \STATE Initialize KV cache $KV \leftarrow [\,]$
% \FOR{$i = 1, \ldots, M$}
%   \STATE Initialize $x^{i}_{t_T} \sim \mathcal{N}(0, I)$
%   \FOR{$j = T, \ldots, 1$}
%     \STATE Set $\hat{x}^{i}_{0} \leftarrow G_{\theta}(x^{i}_{t_j}; t_j, KV)$
%     \IF{$j = 1$}
%       \STATE $X_{\theta}.\mathrm{append}(\hat{x}^{i}_{0})$
%       \STATE Cache $kv_i \leftarrow G^{KV}_{\theta}(\hat{x}^{i}_{0}; 0, KV)$
%       \IF{$|KV| = L$}
%         \STATE $KV.\mathrm{pop}(0)$ \COMMENT{Cache eviction}
%       \ENDIF
%       \STATE $KV.\mathrm{append}(kv_i)$
%     \ELSE
%       \STATE Sample $\epsilon \sim \mathcal{N}(0, I)$
%       \STATE Set $x^{i}_{t_{j-1}} \leftarrow \Psi(\hat{x}^{i}_{0}, \epsilon, t_{j-1})$
%     \ENDIF
%   \ENDFOR
% \ENDFOR
% \STATE \textbf{return} $X_{\theta}$
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[t]
% \caption{Autoregressive Diffusion Inference with Rolling KV Cache in Sparse Forcing}
% \label{alg:sparse_forcing_infer}
% \begin{algorithmic}[1]
% \REQUIRE KV cache budget $L$ (in frames / blocks)
% \REQUIRE Denoise timesteps $\{t_1, \ldots, t_T\}$
% \REQUIRE Number of generated frames $M$
% \REQUIRE AR diffusion model $G_{\theta}$ (returns KV embeddings via $G^{KV}_{\theta}$)
% % {\color{blue}\REQUIRE Block shape $(C_t,C_h,C_w)$ and persistent budget $C$}
% % {\color{blue}\REQUIRE Block reshape operator $\mathrm{BlockReshape}(\cdot)$ (Alg.~\ref{alg:block_reshape})}
% % {\color{blue}\REQUIRE Block compression operators $\phi_K,\phi_V$ and coarse scoring $\psi(\cdot)$}

% \STATE Initialize model output $X_{\theta} \leftarrow [\,]$
% % \STATE Initialize KV cache $KV \leftarrow [\,]$
% {\color{blue}\STATE Initialize persistent memory $\mathcal{P} \leftarrow [\,]$}
% {\color{blue}\STATE Initialize local KV memory $\mathcal{L} \leftarrow [\,]$}

% \FOR{$i = 1, \ldots, M$}
%   \STATE Initialize $x^{i}_{t_T} \sim \mathcal{N}(0, I)$
%   \FOR{$j = T, \ldots, 1$}
%     \STATE Set $\hat{x}^{i}_{0} \leftarrow G_{\theta}(x^{i}_{t_j}; t_j, \mathcal{P}, \mathcal{L})$
%     % {\color{blue}\STATE Construct effective KV view: $KV_{\text{eff}} \leftarrow \mathrm{Assemble}(KV,\mathcal{P})$}
%     % {\color{blue}\STATE $\hat{x}^{i}_{0} \leftarrow G_{\theta}(x^{i}_{t_j}; t_j, KV_{\text{eff}})$ \COMMENT{Sparse Forcing attention}}
%     \IF{$j = 1$}
%       \STATE $X_{\theta}.\mathrm{append}(\hat{x}^{i}_{0})$
%       \STATE Cache $\mathcal{P}, \mathcal{L} \leftarrow G^{KV}_{\theta}(\hat{x}^{i}_{0}; 0, \mathcal{P}, \mathcal{L})$
      
%       % {\color{blue}\STATE $kv_i^{\text{blk}} \leftarrow \mathrm{BlockReshape}(kv_i)$ \COMMENT{locality-preserving layout}}
%       {\color{blue}\STATE $KV.\mathrm{append}(kv_i^{\text{blk}})$}

%       \IF{$|\mathcal{P}| > L_{persist}$}
%         \STATE $\mathcal{L}_{\text{evict}} \leftarrow \mathcal{L}.\mathrm{pop}(0)$ \COMMENT{Cache eviction}
%         {\color{blue}\STATE $\tilde{K} \leftarrow \phi_K(L^{k}_{\text{evict}})$\COMMENT{compress evicted blocks}}
%         {\color{blue}\STATE $\tilde{Q} \leftarrow \phi_K(L^{q})$\COMMENT{compress Q blocks}}
        
%         {\color{blue}\STATE $p \leftarrow \psi(\tilde{Q}, \tilde{K}, \tilde{P})$ \COMMENT{coarse block importance}}
%         {\color{blue}\STATE Aggregate across all Q to have $P_{aggr}$}
%         {\color{blue}\STATE $\mathcal{P} \leftarrow \mathrm{Top}\text{-}C\ \mathrm{Retain}(\mathcal{P} \cup \{(\tilde{K},\tilde{V})\};\, p)$ \COMMENT{update persistent anchors}}
%       \ENDIF
      
%     \ELSE
%       \STATE Sample $\epsilon \sim \mathcal{N}(0, I)$
%       \STATE Set $x^{i}_{t_{j-1}} \leftarrow \Psi(\hat{x}^{i}_{0}, \epsilon, t_{j-1})$
      
%       {\color{blue}\STATE \COMMENT{At intermediate denoising steps, only current blocks are refreshed; $\mathcal{P}$ is shared across $j$}}
%     \ENDIF
    
%   \ENDFOR
% \ENDFOR
% \STATE \textbf{return} $X_{\theta}$
% \end{algorithmic}
% \end{algorithm}



\begin{algorithm}[t]
\caption{Autoregressive Diffusion Inference with Rolling KV Cache in Sparse Forcing}
\label{alg:sparse_forcing_infer}
\begin{algorithmic}[1]
\REQUIRE KV cache budget $L$ (in frames / blocks)
\REQUIRE Denoise timesteps $\{t_1, \ldots, t_T\}$
\REQUIRE Number of generated frames $M$
\REQUIRE AR diffusion model $G_{\theta}$ (returns KV embeddings via $G^{KV}_{\theta}$)
% {\color{blue}\REQUIRE Block shape $(C_t,C_h,C_w)$ and persistent budget $C$}
% {\color{blue}\REQUIRE Block reshape operator $\mathrm{BlockReshape}(\cdot)$ (Alg.~\ref{alg:block_reshape})}
% {\color{blue}\REQUIRE Block compression operators $\phi_K,\phi_V$ and coarse scoring $\psi(\cdot)$}
\STATE Initialize model output $X_{\theta} \leftarrow [\,]$
{\color{blue}\STATE Initialize persistent memory $\mathcal{P} \leftarrow [\,]$ \COMMENT{capacity $C$ blocks}}
{\color{blue}\STATE Initialize local KV window $\mathcal{L} \leftarrow [\,]$ \COMMENT{capacity $L_{\text{local}}$ frames/blocks}}

\FOR{$i = 1, \ldots, M$}
  \STATE Initialize $x^{i}_{t_T} \sim \mathcal{N}(0, I)$
  \FOR{$j = T, \ldots, 1$}
    \STATE Set $\hat{x}^{i}_{0} \leftarrow G_{\theta}(x^{i}_{t_j}; t_j, \mathcal{P}, \mathcal{L})$
    \IF{$j = 1$}
      \STATE $X_{\theta}.\mathrm{append}(\hat{x}^{i}_{0})$
      {\color{blue}\STATE $kv_i \leftarrow G^{KV}_{\theta}(\hat{x}^{i}_{0}; 0)$ \COMMENT{KV for the new denoised frame}}
      {\color{blue}\STATE $\mathcal{L}.\mathrm{append}(kv_i)$ \COMMENT{push into local window}}

      {\color{blue}\IF{$|\mathcal{L}| > L_{\text{local}}$}}
        {\color{blue}\STATE $kv_{\text{evict}} \leftarrow \mathcal{L}.\mathrm{pop}(0)$ \COMMENT{evict oldest local KV}}
        {\color{blue}\STATE $(\tilde{K},\tilde{V}) \leftarrow (\phi_K(kv_{\text{evict}}),\phi_V(kv_{\text{evict}}))$ \COMMENT{block compression}}
        {\color{blue}\STATE $\tilde{Q} \leftarrow \phi_Q(\mathcal{L})$ \COMMENT{compress current local queries for scoring}}
        {\color{blue}\STATE $p \leftarrow \psi(\tilde{Q}, \tilde{K})$ \COMMENT{coarse importance score}}
        {\color{blue}\STATE $\mathcal{P} \leftarrow \mathrm{Top}\text{-}C\ \mathrm{Retain}(\mathcal{P} \cup \{(\tilde{K},\tilde{V})\};\, p)$}
      {\color{blue}\ENDIF}

    \ELSE
      \STATE Sample $\epsilon \sim \mathcal{N}(0, I)$
      \STATE Set $x^{i}_{t_{j-1}} \leftarrow \Psi(\hat{x}^{i}_{0}, \epsilon, t_{j-1})$
    \ENDIF
  \ENDFOR
\ENDFOR
\STATE \textbf{return} $X_{\theta}$
\end{algorithmic}
\end{algorithm}

==> tables/long_qc_old.tex <==
\begin{table*}[t]
  \centering
  \caption{Comparison with relevant baselines on long-horizon generation.}
  \label{tab:long_video_comparison_baselines}

  \footnotesize
  \setlength{\tabcolsep}{4.5pt}
  \renewcommand{\arraystretch}{1.08}

  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}X c c c c c}
    \toprule
    \multirow{2}{*}{Model} &
    \multirow{2}{*}{\makecell[c]{Throughput\\(FPS) $\uparrow$}} &
    \multirow{2}{*}{\makecell[c]{Latency\\(s) $\downarrow$}} &
    \multicolumn{3}{c}{Evaluation scores $\uparrow$} \\
    \cmidrule(lr){4-6}
    & & & Total & Quality & Semantic \\
    \midrule

    \multicolumn{6}{l}{\textit{20-second length video}} \\
    Self Forcing &
    15.1 & -- &
    82.09 & 82.48 & 80.51 \\

    \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344}^{\diamond} &
    \SR 18.1 & \SR -- &
    \SR \textcolor{BestTxt}{\textbf{82.77}} &
    \SR \textcolor{BestTxt}{\textbf{83.26}} &
    \SR 80.82 \\

    \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344}^{\blacklozenge} &
    \SR 18.1 & \SR -- &
    \SR 82.68 & \SR 83.13 &
    \SR \textcolor{BestTxt}{\textbf{80.87}} \\

    \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_188}^{\diamond} &
    \SR -- & \SR -- &
    \SR -- &
    \SR -- &
    \SR -- \\

    \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_188}^{\blacklozenge} &
    \SR -- & \SR -- &
    \SR -- & \SR -- &
    \SR -- \\
    
    \midrule

    \multicolumn{6}{l}{\textit{1-minute length video}} \\
    Self Forcing & 
    \SR -- & \SR -- &
    \SR 78.93 & 79.48 & 76.70 \\

    \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344}^{\diamond} &
    \SR -- & \SR -- &
    \SR 81.96 & 82.25 & 80.82 \\

    \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344}^{\blacklozenge} &
    \SR -- & \SR -- &
    \SR 81.67 & 82.17 & 79.67 \\

    \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_188}^{\diamond} &
    \SR -- & \SR -- &
    \SR -- & -- & -- \\

    \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_188}^{\blacklozenge} &
    \SR -- & \SR -- &
    \SR -- & -- & -- \\
    
    \bottomrule
  \end{tabularx}
\end{table*}

% Semantic Score	0.767	0.8082	0.7967
% Quality Score	0.7948	0.8225	0.8217
% Total Vbench Score	0.7893	0.8196	0.8167


% % ===== Preamble (must have) =====
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{makecell}
% % \usepackage[table]{xcolor}
% % \usepackage{tabularx}
% % \usepackage{array}
% % \definecolor{SparseRow}{HTML}{FFF6E5}
% % \definecolor{BestTxt}{HTML}{1F4E79}

% % helper: color one full row cell-by-cell (prevents "broken" rowcolor in tabularx)
% \newcommand{\SR}{\cellcolor{SparseRow}}

% \begin{table*}[t]
%   \centering
%   \caption{Comparison with relevant baselines. We compare Self Forcing with representative
%   open-source video generation models of similar parameter sizes and resolutions.}
%   \label{tab:long_video_comparison_baselines}

%   \footnotesize
%   \setlength{\tabcolsep}{3.5pt}
%   \renewcommand{\arraystretch}{1.10}

%   \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}X c c c c c c c}
%     \toprule
%     \multirow{2}{*}{Model} &
%     \multirow{2}{*}{\#Params} &
%     \multirow{2}{*}{Resolution} &
%     \multirow{2}{*}{\makecell[c]{Throughput\\(FPS) $\uparrow$}} &
%     \multirow{2}{*}{\makecell[c]{Latency\\(s) $\downarrow$}} &
%     \multicolumn{3}{c}{Evaluation scores $\uparrow$} \\
%     \cmidrule(lr){6-8}
%     & & & & & Total & Quality & Semantic \\
%     \midrule

%     % \multicolumn{8}{l}{\textbf{Diffusion models}} \\
%     % LTX-Video [24] & 1.9B & $768{\times}512$ & 8.98 & 13.5 & 80.00 & 82.30 & 70.79 \\
%     % Wan2.1 [83]    & 1.3B & $832{\times}480$ & 0.78 & 103  & 84.26 & 85.30 & 80.09 \\
%     % \midrule

%     % \multicolumn{8}{l}{\textbf{Chunk-wise autoregressive models}} \\
%     % SkyReels-V2 [10] & 1.3B & $960{\times}540$ & 0.49 & 112 & 82.67 & 84.70 & 74.53 \\
%     % MAGI-1 [69]      & 4.5B & $832{\times}480$ & 0.19 & 282 & 79.18 & 82.04 & 67.74 \\
%     % CausVid [100]$^{*}$ & 1.3B & $832{\times}480$ & 17.0 & 0.69 & 81.20 & 84.05 & 69.80 \\
%     % \midrule

%     \multicolumn{8}{l}{\textit{20-second length video}$^{\ddagger}$} \\
%     Self Forcing &
%     1.3B & \makecell[c]{$832{\times}512$} & 15.1 & -- &
%     82.09 & 82.48 & 80.51 \\

%     \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344} &
%     \SR 1.3B & \SR \makecell[c]{$832{\times}512$} & \SR 18.1 & \SR -- &
%     \SR \textcolor{BestTxt}{\textbf{82.77}} &
%     \SR \textcolor{BestTxt}{\textbf{83.26}} &
%     \SR 80.82 \\

%     \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344}-aware training &
%     \SR 1.3B & \SR \makecell[c]{$832{\times}512$} & \SR 18.1 & \SR -- &
%     \SR 82.68 & \SR 83.13 & \SR \textcolor{BestTxt}{\textbf{80.87}} \\
%     \midrule

%     \multicolumn{8}{l}{\textit{1-minute length video}$^{\ddagger}$} \\
%     Self Forcing &
%     1.3B & \makecell[c]{$832{\times}512$} & -- & -- &
%     \multicolumn{3}{c}{\textit{TBD}} \\

%     \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344} &
%     \SR 1.3B & \SR \makecell[c]{$832{\times}512$} & \SR -- & \SR -- &
%     \SR \multicolumn{3}{c}{\textit{TBD}} \\

%     \SR Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344}-aware training &
%     \SR 1.3B & \SR \makecell[c]{$832{\times}512$} & \SR -- & \SR -- &
%     \SR \multicolumn{3}{c}{\textit{TBD}} \\
%     % \midrule

%     % \multicolumn{8}{l}{\textbf{Autoregressive}$^{\dagger}$} \\
%     % NOVA [13]         & 0.6B & $768{\times}480$ & 0.88 & 4.1 & 80.12 & 80.39 & 79.05 \\
%     % Pyramid Flow [33] & 2B   & $640{\times}384$ & 6.7  & 2.5 & 81.72 & 84.74 & 69.62 \\
%     \bottomrule
%   \end{tabularx}

%   % \vspace{2pt}
%   % {\scriptsize
%   % $^{*}$ We compare with the official implementation of CausVid that uses the same base model (Wan-1.3B). \\
%   % $^{\dagger}$ The distinction of AR/non-AR applies to the temporal dimension. \\
%   % $^{\ddagger}$ Long-horizon results use a DMD checkpoint; scores are multiplied by $100$ for consistency with the main table; FPS/latency are not reported (marked as “--”).
%   % }
% \end{table*}


==> tables/partial_kernel_eval.tex <==
\begin{table*}[htbp]
\centering
\caption{Complete Sparse Attention Kernel Benchmark Results. All 480 configurations tested.}
\label{tab:kernel_benchmark_full}
\footnotesize
\begin{tabular}{@{}ccccc|cc|c@{}}
\toprule
topK (\%) & $C$ & $L/C$ & $P/L$ & KV & Sparse (ms) & FA2 (ms) & Speedup \\
\midrule
% --- rows here ---
\benchrow{6.25}{2K}{1}{0.0}{2K}{\pmnum{0.41}{0.01}}{\pmnum{0.17}{0.00}}{0.42$\times$}
\benchrow{6.25}{2K}{1}{0.2}{3K}{\pmnum{0.41}{0.00}}{\pmnum{0.20}{0.00}}{0.49$\times$}
\benchrow{6.25}{2K}{1}{0.5}{4K}{\pmnum{0.43}{0.00}}{\pmnum{0.23}{0.00}}{0.55$\times$}
\benchrow{6.25}{2K}{1}{1.0}{5K}{\pmnum{0.49}{0.01}}{\pmnum{0.30}{0.00}}{0.61$\times$}
\benchrow{6.25}{2K}{1}{2.0}{8K}{\pmnum{0.59}{0.00}}{\pmnum{0.41}{0.00}}{0.70$\times$}
\benchrow{6.25}{2K}{1}{4.0}{13K}{\pmnum{0.80}{0.00}}{\pmnum{0.69}{0.03}}{0.86$\times$}

\benchrow{6.25}{2K}{2}{0.0}{5K}{\pmnum{0.42}{0.00}}{\pmnum{0.32}{0.00}}{0.76$\times$}
\benchrow{6.25}{2K}{2}{0.2}{6K}{\pmnum{0.46}{0.00}}{\pmnum{0.37}{0.00}}{0.80$\times$}
\benchrow{6.25}{2K}{2}{0.5}{8K}{\pmnum{0.51}{0.00}}{\pmnum{0.42}{0.00}}{0.83$\times$}
\benchrow{6.25}{2K}{2}{1.0}{10K}{\pmnum{0.62}{0.01}}{\pmnum{0.54}{0.00}}{0.87$\times$}
\benchrow{6.25}{2K}{2}{2.0}{16K}{\pmnum{0.84}{0.00}}{\pmnum{0.86}{0.00}}{1.03$\times$}
\benchrow{6.25}{2K}{2}{4.0}{26K}{\pmnum{1.31}{0.01}}{\pmnum{1.42}{0.03}}{1.08$\times$}

\benchrow{6.25}{2K}{4}{0.0}{10K}{\pmnum{0.49}{0.01}}{\pmnum{0.58}{0.00}}{1.19$\times$}
\benchrow{6.25}{2K}{4}{0.2}{13K}{\pmnum{0.58}{0.01}}{\pmnum{0.67}{0.01}}{1.16$\times$}
\benchrow{6.25}{2K}{4}{0.5}{16K}{\pmnum{0.68}{0.01}}{\pmnum{0.79}{0.00}}{1.16$\times$}
\benchrow{6.25}{2K}{4}{1.0}{21K}{\pmnum{0.91}{0.00}}{\pmnum{1.10}{0.00}}{1.20$\times$}
\benchrow{6.25}{2K}{4}{2.0}{32K}{\pmnum{1.38}{0.01}}{\pmnum{1.72}{0.00}}{1.25$\times$}
\benchrow{6.25}{2K}{4}{4.0}{53K}{\pmnum{2.30}{0.01}}{\pmnum{2.90}{0.01}}{1.26$\times$}

\benchrow{6.25}{2K}{8}{0.0}{21K}{\pmnum{0.63}{0.01}}{\pmnum{1.10}{0.03}}{1.73$\times$}
\benchrow{6.25}{2K}{8}{0.2}{26K}{\pmnum{0.83}{0.01}}{\pmnum{1.49}{0.01}}{1.81$\times$}
\benchrow{6.25}{2K}{8}{0.5}{32K}{\pmnum{1.07}{0.01}}{\pmnum{1.71}{0.01}}{1.60$\times$}
\benchrow{6.25}{2K}{8}{1.0}{43K}{\pmnum{1.51}{0.01}}{\pmnum{2.29}{0.00}}{1.51$\times$}
\benchrow{6.25}{2K}{8}{2.0}{64K}{\pmnum{2.41}{0.00}}{\pmnum{3.49}{0.02}}{1.45$\times$}
\benchrow{6.25}{2K}{8}{4.0}{107K}{\pmnum{4.62}{0.06}}{\pmnum{5.74}{0.02}}{1.24$\times$}

\benchrow{6.25}{5K}{1}{0.0}{5K}{\pmnum{0.44}{0.00}}{\pmnum{0.56}{0.00}}{1.28$\times$}
\benchrow{6.25}{5K}{1}{0.2}{6K}{\pmnum{0.52}{0.01}}{\pmnum{0.67}{0.00}}{1.29$\times$}
\benchrow{6.25}{5K}{1}{0.5}{8K}{\pmnum{0.62}{0.02}}{\pmnum{0.80}{0.00}}{1.29$\times$}
\benchrow{6.25}{5K}{1}{1.0}{10K}{\pmnum{0.81}{0.00}}{\pmnum{1.17}{0.01}}{1.45$\times$}
\benchrow{6.25}{5K}{1}{2.0}{16K}{\pmnum{1.27}{0.01}}{\pmnum{1.79}{0.01}}{1.41$\times$}
\benchrow{6.25}{5K}{1}{4.0}{26K}{\pmnum{2.06}{0.01}}{\pmnum{2.89}{0.02}}{1.40$\times$}

\benchrow{6.25}{5K}{2}{0.0}{10K}{\pmnum{0.51}{0.01}}{\pmnum{1.09}{0.01}}{2.1$\times$}
\benchrow{6.25}{5K}{2}{0.2}{13K}{\pmnum{0.69}{0.00}}{\pmnum{1.34}{0.04}}{1.94$\times$}
\benchrow{6.25}{5K}{2}{0.5}{16K}{\pmnum{0.91}{0.01}}{\pmnum{1.72}{0.00}}{1.90$\times$}
\benchrow{6.25}{5K}{2}{1.0}{21K}{\pmnum{1.32}{0.00}}{\pmnum{2.28}{0.00}}{1.72$\times$}
\benchrow{6.25}{5K}{2}{2.0}{32K}{\pmnum{2.15}{0.01}}{\pmnum{3.46}{0.02}}{1.61$\times$}
\benchrow{6.25}{5K}{2}{4.0}{53K}{\pmnum{3.89}{0.04}}{\pmnum{5.73}{0.04}}{1.47$\times$}

\benchrow{6.25}{5K}{4}{0.0}{21K}{\pmnum{0.65}{0.01}}{\pmnum{2.08}{0.06}}{3.2$\times$}
\benchrow{6.25}{5K}{4}{0.2}{26K}{\pmnum{1.04}{0.00}}{\pmnum{3.02}{0.12}}{2.9$\times$}
\benchrow{6.25}{5K}{4}{0.5}{32K}{\pmnum{1.49}{0.01}}{\pmnum{3.40}{0.09}}{2.3$\times$}
\benchrow{6.25}{5K}{4}{1.0}{43K}{\pmnum{2.26}{0.01}}{\pmnum{4.79}{0.07}}{2.1$\times$}
\benchrow{6.25}{5K}{4}{2.0}{64K}{\pmnum{4.22}{0.04}}{\pmnum{6.58}{0.02}}{1.56$\times$}
\benchrow{6.25}{5K}{4}{4.0}{107K}{\pmnum{7.75}{0.08}}{\pmnum{11.07}{0.19}}{1.43$\times$}

% \benchrow{6.25}{5K}{8}{0.0}{43K}{\pmnum{0.92}{0.00}}{\pmnum{4.66}{0.03}}{\textbf{5.1$\times$}}
% \benchrow{6.25}{5K}{8}{0.2}{53K}{\pmnum{1.76}{0.00}}{\pmnum{5.72}{0.00}}{3.3$\times$}
% \benchrow{6.25}{5K}{8}{0.5}{64K}{\pmnum{2.59}{0.01}}{\pmnum{6.82}{0.16}}{2.6$\times$}
% \benchrow{6.25}{5K}{8}{1.0}{86K}{\pmnum{4.18}{0.01}}{\pmnum{9.03}{0.09}}{2.2$\times$}
% \benchrow{6.25}{5K}{8}{2.0}{129K}{\pmnum{7.94}{0.25}}{\pmnum{13.45}{0.14}}{1.69$\times$}
% \benchrow{6.25}{5K}{8}{4.0}{215K}{\pmnum{15.87}{1.22}}{\pmnum{22.35}{0.38}}{1.41$\times$}

% \benchrow{6.25}{10K}{1}{0.0}{10K}{\pmnum{0.56}{0.01}}{\pmnum{2.13}{0.07}}{3.8$\times$}
% \benchrow{6.25}{10K}{1}{0.2}{13K}{\pmnum{0.92}{0.00}}{\pmnum{2.80}{0.00}}{3.0$\times$}
% \benchrow{6.25}{10K}{1}{0.5}{16K}{\pmnum{1.30}{0.01}}{\pmnum{3.53}{0.04}}{2.7$\times$}
% \benchrow{6.25}{10K}{1}{1.0}{21K}{\pmnum{2.10}{0.02}}{\pmnum{4.78}{0.09}}{2.3$\times$}
% \benchrow{6.25}{10K}{1}{2.0}{32K}{\pmnum{3.88}{0.07}}{\pmnum{6.89}{0.09}}{1.78$\times$}
% \benchrow{6.25}{10K}{1}{4.0}{53K}{\pmnum{7.10}{0.44}}{\pmnum{11.13}{0.07}}{1.57$\times$}

% \benchrow{6.25}{10K}{2}{0.0}{21K}{\pmnum{0.75}{0.00}}{\pmnum{4.53}{0.02}}{\textbf{6.1$\times$}}
% \benchrow{6.25}{10K}{2}{0.2}{26K}{\pmnum{1.52}{0.01}}{\pmnum{5.70}{0.01}}{3.8$\times$}
% \benchrow{6.25}{10K}{2}{0.5}{32K}{\pmnum{2.34}{0.03}}{\pmnum{6.89}{0.00}}{2.9$\times$}
% \benchrow{6.25}{10K}{2}{1.0}{43K}{\pmnum{4.20}{0.08}}{\pmnum{8.74}{0.13}}{2.1$\times$}
% \benchrow{6.25}{10K}{2}{2.0}{64K}{\pmnum{7.60}{0.10}}{\pmnum{13.15}{0.12}}{1.73$\times$}
% \benchrow{6.25}{10K}{2}{4.0}{107K}{\pmnum{14.89}{0.65}}{\pmnum{22.07}{0.29}}{1.48$\times$}

% \benchrow{6.25}{10K}{4}{0.0}{43K}{\pmnum{1.17}{0.01}}{\pmnum{8.72}{0.07}}{\textbf{7.4$\times$}}
% \benchrow{6.25}{10K}{4}{0.2}{53K}{\pmnum{2.68}{0.01}}{\pmnum{11.65}{0.42}}{4.3$\times$}
% \benchrow{6.25}{10K}{4}{0.5}{64K}{\pmnum{4.62}{0.14}}{\pmnum{13.11}{0.23}}{2.8$\times$}
% \benchrow{6.25}{10K}{4}{1.0}{86K}{\pmnum{8.43}{0.34}}{\pmnum{17.64}{0.25}}{2.1$\times$}
% \benchrow{6.25}{10K}{4}{2.0}{129K}{\pmnum{15.53}{0.38}}{\pmnum{26.67}{0.36}}{1.72$\times$}
% \benchrow{6.25}{10K}{4}{4.0}{215K}{\pmnum{29.59}{0.92}}{\pmnum{45.45}{0.45}}{1.54$\times$}

% \benchrow{6.25}{10K}{8}{0.0}{86K}{\pmnum{2.16}{0.01}}{\pmnum{17.36}{0.07}}{\textbf{8.0$\times$}}
% \benchrow{6.25}{10K}{8}{0.2}{107K}{\pmnum{5.20}{0.01}}{\pmnum{22.71}{0.36}}{4.4$\times$}
% \benchrow{6.25}{10K}{8}{0.5}{129K}{\pmnum{9.92}{0.33}}{\pmnum{26.51}{0.33}}{2.7$\times$}
% \benchrow{6.25}{10K}{8}{1.0}{172K}{\pmnum{16.84}{0.37}}{\pmnum{35.13}{0.19}}{2.1$\times$}
% \benchrow{6.25}{10K}{8}{2.0}{258K}{\pmnum{29.96}{0.81}}{\pmnum{54.66}{0.74}}{1.82$\times$}
% \benchrow{6.25}{10K}{8}{4.0}{430K}{\pmnum{58.95}{1.16}}{\pmnum{89.71}{0.74}}{1.52$\times$}

% \benchrow{6.25}{21K}{1}{0.0}{21K}{\pmnum{0.94}{0.01}}{\pmnum{9.05}{0.01}}{\textbf{9.6$\times$}}
% \benchrow{6.25}{21K}{1}{0.2}{26K}{\pmnum{2.37}{0.02}}{\pmnum{11.08}{0.07}}{4.7$\times$}
% \benchrow{6.25}{21K}{1}{0.5}{32K}{\pmnum{4.13}{0.08}}{\pmnum{13.20}{0.10}}{3.2$\times$}
% \benchrow{6.25}{21K}{1}{1.0}{43K}{\pmnum{8.31}{0.25}}{\pmnum{17.70}{0.18}}{2.1$\times$}
% \benchrow{6.25}{21K}{1}{2.0}{64K}{\pmnum{15.35}{0.67}}{\pmnum{26.91}{0.27}}{1.75$\times$}
% \benchrow{6.25}{21K}{1}{4.0}{107K}{\pmnum{28.38}{0.47}}{\pmnum{44.94}{0.70}}{1.58$\times$}

% \benchrow{6.25}{21K}{2}{0.0}{43K}{\pmnum{1.72}{0.00}}{\pmnum{17.59}{0.10}}{\textbf{10.2$\times$}}
% \benchrow{6.25}{21K}{2}{0.2}{53K}{\pmnum{4.67}{0.02}}{\pmnum{22.42}{0.38}}{4.8$\times$}
% \benchrow{6.25}{21K}{2}{0.5}{64K}{\pmnum{8.88}{0.21}}{\pmnum{26.74}{0.37}}{3.0$\times$}
% \benchrow{6.25}{21K}{2}{1.0}{86K}{\pmnum{15.02}{0.37}}{\pmnum{35.16}{0.35}}{2.3$\times$}
% \benchrow{6.25}{21K}{2}{2.0}{129K}{\pmnum{28.92}{0.71}}{\pmnum{54.58}{0.60}}{1.89$\times$}
% \benchrow{6.25}{21K}{2}{4.0}{215K}{\pmnum{55.66}{1.41}}{\pmnum{89.85}{0.85}}{1.61$\times$}

% \benchrow{6.25}{21K}{4}{0.0}{86K}{\pmnum{3.24}{0.01}}{\pmnum{35.96}{0.21}}{\textbf{11.1$\times$}}
% \benchrow{6.25}{21K}{4}{0.2}{107K}{\pmnum{10.75}{0.53}}{\pmnum{44.84}{0.58}}{4.2$\times$}
% \benchrow{6.25}{21K}{4}{0.5}{129K}{\pmnum{16.26}{0.41}}{\pmnum{54.40}{0.67}}{3.3$\times$}
% \benchrow{6.25}{21K}{4}{1.0}{172K}{\pmnum{30.25}{0.44}}{\pmnum{71.98}{1.43}}{2.4$\times$}
% \benchrow{6.25}{21K}{4}{2.0}{258K}{\pmnum{56.89}{1.56}}{\pmnum{108.01}{0.72}}{1.90$\times$}
% \benchrow{6.25}{21K}{4}{4.0}{430K}{\pmnum{120.19}{5.21}}{\pmnum{178.59}{1.64}}{1.49$\times$}

% \benchrow{6.25}{21K}{8}{0.0}{172K}{\pmnum{7.63}{0.09}}{\pmnum{71.57}{0.62}}{\textbf{9.4$\times$}}
% \benchrow{6.25}{21K}{8}{0.2}{215K}{\pmnum{19.40}{0.64}}{\pmnum{89.56}{0.72}}{4.6$\times$}
% \benchrow{6.25}{21K}{8}{0.5}{258K}{\pmnum{33.33}{0.53}}{\pmnum{107.11}{0.53}}{3.2$\times$}
% \benchrow{6.25}{21K}{8}{1.0}{344K}{\pmnum{60.30}{1.26}}{\pmnum{142.72}{0.95}}{2.4$\times$}
% \benchrow{6.25}{21K}{8}{2.0}{516K}{\pmnum{118.01}{3.67}}{\pmnum{214.48}{2.15}}{1.82$\times$}
% \benchrow{6.25}{21K}{8}{4.0}{860K}{\pmnum{247.57}{9.52}}{\pmnum{361.98}{2.90}}{1.46$\times$}

\midrule
% ============================
% topK = 12.50
% ============================
\benchrow{12.50}{2K}{1}{0.0}{2K}{\pmnum{0.39}{0.01}}{\pmnum{0.18}{0.00}}{0.45$\times$}
\benchrow{12.50}{2K}{1}{0.2}{3K}{\pmnum{0.41}{0.01}}{\pmnum{0.20}{0.00}}{0.49$\times$}
\benchrow{12.50}{2K}{1}{0.5}{4K}{\pmnum{0.44}{0.01}}{\pmnum{0.23}{0.00}}{0.54$\times$}
\benchrow{12.50}{2K}{1}{1.0}{5K}{\pmnum{0.48}{0.00}}{\pmnum{0.30}{0.01}}{0.62$\times$}
\benchrow{12.50}{2K}{1}{2.0}{8K}{\pmnum{0.59}{0.01}}{\pmnum{0.42}{0.01}}{0.71$\times$}
\benchrow{12.50}{2K}{1}{4.0}{13K}{\pmnum{0.82}{0.01}}{\pmnum{0.67}{0.00}}{0.82$\times$}

\benchrow{12.50}{2K}{2}{0.0}{5K}{\pmnum{0.42}{0.00}}{\pmnum{0.30}{0.01}}{0.71$\times$}
\benchrow{12.50}{2K}{2}{0.2}{6K}{\pmnum{0.47}{0.01}}{\pmnum{0.36}{0.00}}{0.77$\times$}
\benchrow{12.50}{2K}{2}{0.5}{8K}{\pmnum{0.52}{0.01}}{\pmnum{0.42}{0.00}}{0.81$\times$}
\benchrow{12.50}{2K}{2}{1.0}{10K}{\pmnum{0.63}{0.00}}{\pmnum{0.55}{0.00}}{0.87$\times$}
\benchrow{12.50}{2K}{2}{2.0}{16K}{\pmnum{0.87}{0.01}}{\pmnum{0.86}{0.00}}{1.00$\times$}
\benchrow{12.50}{2K}{2}{4.0}{26K}{\pmnum{1.34}{0.01}}{\pmnum{1.42}{0.00}}{1.06$\times$}

% \benchrow{12.50}{2K}{4}{0.0}{10K}{\pmnum{0.51}{0.01}}{\pmnum{0.60}{0.02}}{1.18$\times$}
% \benchrow{12.50}{2K}{4}{0.2}{13K}{\pmnum{0.61}{0.01}}{\pmnum{0.68}{0.01}}{1.12$\times$}
% \benchrow{12.50}{2K}{4}{0.5}{16K}{\pmnum{0.71}{0.01}}{\pmnum{0.81}{0.00}}{1.14$\times$}
% \benchrow{12.50}{2K}{4}{1.0}{21K}{\pmnum{0.96}{0.01}}{\pmnum{1.16}{0.01}}{1.21$\times$}
% \benchrow{12.50}{2K}{4}{2.0}{32K}{\pmnum{1.44}{0.04}}{\pmnum{1.73}{0.00}}{1.20$\times$}
% \benchrow{12.50}{2K}{4}{4.0}{53K}{\pmnum{2.35}{0.01}}{\pmnum{2.94}{0.01}}{1.25$\times$}

% \benchrow{12.50}{2K}{8}{0.0}{21K}{\pmnum{0.65}{0.00}}{\pmnum{1.14}{0.00}}{1.76$\times$}
% \benchrow{12.50}{2K}{8}{0.2}{26K}{\pmnum{0.87}{0.00}}{\pmnum{1.41}{0.00}}{1.62$\times$}
% \benchrow{12.50}{2K}{8}{0.5}{32K}{\pmnum{1.10}{0.01}}{\pmnum{1.72}{0.01}}{1.56$\times$}
% \benchrow{12.50}{2K}{8}{1.0}{43K}{\pmnum{1.56}{0.01}}{\pmnum{2.31}{0.00}}{1.48$\times$}
% \benchrow{12.50}{2K}{8}{2.0}{64K}{\pmnum{2.49}{0.01}}{\pmnum{3.55}{0.02}}{1.43$\times$}
% \benchrow{12.50}{2K}{8}{4.0}{107K}{\pmnum{4.92}{0.04}}{\pmnum{5.82}{0.07}}{1.18$\times$}

% \benchrow{12.50}{5K}{1}{0.0}{5K}{\pmnum{0.46}{0.01}}{\pmnum{0.62}{0.02}}{1.34$\times$}
% \benchrow{12.50}{5K}{1}{0.2}{6K}{\pmnum{0.55}{0.00}}{\pmnum{0.70}{0.00}}{1.26$\times$}
% \benchrow{12.50}{5K}{1}{0.5}{8K}{\pmnum{0.64}{0.01}}{\pmnum{0.81}{0.00}}{1.26$\times$}
% \benchrow{12.50}{5K}{1}{1.0}{10K}{\pmnum{0.86}{0.01}}{\pmnum{1.11}{0.00}}{1.30$\times$}
% \benchrow{12.50}{5K}{1}{2.0}{16K}{\pmnum{1.28}{0.01}}{\pmnum{1.74}{0.00}}{1.36$\times$}
% \benchrow{12.50}{5K}{1}{4.0}{26K}{\pmnum{2.11}{0.01}}{\pmnum{2.95}{0.03}}{1.40$\times$}

% \benchrow{12.50}{5K}{2}{0.0}{10K}{\pmnum{0.57}{0.02}}{\pmnum{1.09}{0.01}}{1.92$\times$}
% \benchrow{12.50}{5K}{2}{0.2}{13K}{\pmnum{0.76}{0.01}}{\pmnum{1.35}{0.01}}{1.78$\times$}
% \benchrow{12.50}{5K}{2}{0.5}{16K}{\pmnum{0.97}{0.01}}{\pmnum{1.68}{0.01}}{1.74$\times$}
% \benchrow{12.50}{5K}{2}{1.0}{21K}{\pmnum{1.38}{0.01}}{\pmnum{2.32}{0.01}}{1.68$\times$}
% \benchrow{12.50}{5K}{2}{2.0}{32K}{\pmnum{2.21}{0.01}}{\pmnum{3.51}{0.04}}{1.59$\times$}
% \benchrow{12.50}{5K}{2}{4.0}{53K}{\pmnum{4.01}{0.04}}{\pmnum{5.79}{0.03}}{1.44$\times$}

% \benchrow{12.50}{5K}{4}{0.0}{21K}{\pmnum{0.75}{0.01}}{\pmnum{2.33}{0.02}}{3.1$\times$}
% \benchrow{12.50}{5K}{4}{0.2}{26K}{\pmnum{1.16}{0.01}}{\pmnum{3.03}{0.02}}{2.6$\times$}
% \benchrow{12.50}{5K}{4}{0.5}{32K}{\pmnum{1.58}{0.02}}{\pmnum{3.55}{0.06}}{2.2$\times$}
% \benchrow{12.50}{5K}{4}{1.0}{43K}{\pmnum{2.40}{0.01}}{\pmnum{4.68}{0.03}}{1.95$\times$}
% \benchrow{12.50}{5K}{4}{2.0}{64K}{\pmnum{4.34}{0.04}}{\pmnum{6.82}{0.08}}{1.57$\times$}
% \benchrow{12.50}{5K}{4}{4.0}{107K}{\pmnum{7.91}{0.31}}{\pmnum{11.16}{0.10}}{1.41$\times$}

% \benchrow{12.50}{5K}{8}{0.0}{43K}{\pmnum{1.13}{0.01}}{\pmnum{4.60}{0.01}}{4.1$\times$}
% \benchrow{12.50}{5K}{8}{0.2}{53K}{\pmnum{1.94}{0.01}}{\pmnum{6.22}{0.13}}{3.2$\times$}
% \benchrow{12.50}{5K}{8}{0.5}{64K}{\pmnum{2.85}{0.03}}{\pmnum{6.73}{0.07}}{2.4$\times$}
% \benchrow{12.50}{5K}{8}{1.0}{86K}{\pmnum{4.71}{0.02}}{\pmnum{8.91}{0.10}}{1.89$\times$}
% \benchrow{12.50}{5K}{8}{2.0}{129K}{\pmnum{8.26}{0.13}}{\pmnum{13.58}{0.11}}{1.64$\times$}
% \benchrow{12.50}{5K}{8}{4.0}{215K}{\pmnum{16.09}{0.63}}{\pmnum{22.53}{0.51}}{1.40$\times$}

% \benchrow{12.50}{10K}{1}{0.0}{10K}{\pmnum{0.66}{0.01}}{\pmnum{2.23}{0.01}}{3.4$\times$}
% \benchrow{12.50}{10K}{1}{0.2}{13K}{\pmnum{1.02}{0.00}}{\pmnum{2.82}{0.03}}{2.8$\times$}
% \benchrow{12.50}{10K}{1}{0.5}{16K}{\pmnum{1.43}{0.01}}{\pmnum{3.56}{0.02}}{2.5$\times$}
% \benchrow{12.50}{10K}{1}{1.0}{21K}{\pmnum{2.28}{0.04}}{\pmnum{4.81}{0.08}}{2.1$\times$}
% \benchrow{12.50}{10K}{1}{2.0}{32K}{\pmnum{4.09}{0.10}}{\pmnum{6.82}{0.08}}{1.67$\times$}
% \benchrow{12.50}{10K}{1}{4.0}{53K}{\pmnum{7.40}{0.09}}{\pmnum{10.91}{0.11}}{1.47$\times$}

% \benchrow{12.50}{10K}{2}{0.0}{21K}{\pmnum{0.93}{0.01}}{\pmnum{4.47}{0.03}}{4.8$\times$}
% \benchrow{12.50}{10K}{2}{0.2}{26K}{\pmnum{1.68}{0.01}}{\pmnum{5.81}{0.16}}{3.5$\times$}
% \benchrow{12.50}{10K}{2}{0.5}{32K}{\pmnum{2.62}{0.01}}{\pmnum{7.03}{0.04}}{2.7$\times$}
% \benchrow{12.50}{10K}{2}{1.0}{43K}{\pmnum{4.14}{0.02}}{\pmnum{8.84}{0.18}}{2.1$\times$}
% \benchrow{12.50}{10K}{2}{2.0}{64K}{\pmnum{7.64}{0.30}}{\pmnum{13.28}{0.12}}{1.74$\times$}
% \benchrow{12.50}{10K}{2}{4.0}{107K}{\pmnum{15.12}{0.61}}{\pmnum{22.17}{0.39}}{1.47$\times$}

% \benchrow{12.50}{10K}{4}{0.0}{43K}{\pmnum{1.55}{0.00}}{\pmnum{8.74}{0.01}}{\textbf{5.6$\times$}}
% \benchrow{12.50}{10K}{4}{0.2}{53K}{\pmnum{3.18}{0.09}}{\pmnum{11.56}{0.28}}{3.6$\times$}
% \benchrow{12.50}{10K}{4}{0.5}{64K}{\pmnum{5.31}{0.05}}{\pmnum{13.18}{0.14}}{2.5$\times$}
% \benchrow{12.50}{10K}{4}{1.0}{86K}{\pmnum{8.56}{0.33}}{\pmnum{18.09}{0.25}}{2.1$\times$}
% \benchrow{12.50}{10K}{4}{2.0}{129K}{\pmnum{15.70}{0.55}}{\pmnum{26.64}{0.15}}{1.70$\times$}
% \benchrow{12.50}{10K}{4}{4.0}{215K}{\pmnum{29.73}{0.94}}{\pmnum{45.80}{0.22}}{1.54$\times$}

% \benchrow{12.50}{10K}{8}{0.0}{86K}{\pmnum{3.02}{0.01}}{\pmnum{18.03}{0.66}}{\textbf{6.0$\times$}}
% \benchrow{12.50}{10K}{8}{0.2}{107K}{\pmnum{6.46}{0.12}}{\pmnum{22.67}{0.27}}{3.5$\times$}
% \benchrow{12.50}{10K}{8}{0.5}{129K}{\pmnum{10.70}{0.49}}{\pmnum{26.80}{0.23}}{2.5$\times$}
% \benchrow{12.50}{10K}{8}{1.0}{172K}{\pmnum{16.86}{0.51}}{\pmnum{35.67}{0.49}}{2.1$\times$}
% \benchrow{12.50}{10K}{8}{2.0}{258K}{\pmnum{30.57}{0.88}}{\pmnum{54.55}{0.80}}{1.78$\times$}
% \benchrow{12.50}{10K}{8}{4.0}{430K}{\pmnum{59.19}{1.20}}{\pmnum{89.95}{0.88}}{1.52$\times$}

% \benchrow{12.50}{21K}{1}{0.0}{21K}{\pmnum{1.37}{0.00}}{\pmnum{9.05}{0.01}}{\textbf{6.6$\times$}}
% \benchrow{12.50}{21K}{1}{0.2}{26K}{\pmnum{2.85}{0.05}}{\pmnum{11.20}{0.03}}{3.9$\times$}
% \benchrow{12.50}{21K}{1}{0.5}{32K}{\pmnum{4.60}{0.12}}{\pmnum{13.22}{0.08}}{2.9$\times$}
% \benchrow{12.50}{21K}{1}{1.0}{43K}{\pmnum{8.33}{0.32}}{\pmnum{17.88}{0.14}}{2.1$\times$}
% \benchrow{12.50}{21K}{1}{2.0}{64K}{\pmnum{15.27}{0.66}}{\pmnum{26.96}{0.22}}{1.77$\times$}
% \benchrow{12.50}{21K}{1}{4.0}{107K}{\pmnum{28.60}{0.45}}{\pmnum{45.24}{0.47}}{1.58$\times$}

% \benchrow{12.50}{21K}{2}{0.0}{43K}{\pmnum{2.52}{0.02}}{\pmnum{17.51}{0.12}}{\textbf{7.0$\times$}}
% \benchrow{12.50}{21K}{2}{0.2}{53K}{\pmnum{5.40}{0.10}}{\pmnum{22.49}{0.33}}{4.2$\times$}
% \benchrow{12.50}{21K}{2}{0.5}{64K}{\pmnum{10.15}{0.36}}{\pmnum{26.72}{0.31}}{2.6$\times$}
% \benchrow{12.50}{21K}{2}{1.0}{86K}{\pmnum{15.75}{0.58}}{\pmnum{35.38}{0.36}}{2.2$\times$}
% \benchrow{12.50}{21K}{2}{2.0}{129K}{\pmnum{29.20}{0.62}}{\pmnum{54.62}{0.91}}{1.87$\times$}
% \benchrow{12.50}{21K}{2}{4.0}{215K}{\pmnum{56.82}{1.42}}{\pmnum{89.75}{0.73}}{1.58$\times$}

% \benchrow{12.50}{21K}{4}{0.0}{86K}{\pmnum{5.12}{0.11}}{\pmnum{35.87}{0.22}}{\textbf{7.0$\times$}}
% \benchrow{12.50}{21K}{4}{0.2}{107K}{\pmnum{12.39}{0.22}}{\pmnum{44.79}{0.56}}{3.6$\times$}
% \benchrow{12.50}{21K}{4}{0.5}{129K}{\pmnum{18.21}{0.64}}{\pmnum{54.35}{0.46}}{3.0$\times$}
% \benchrow{12.50}{21K}{4}{1.0}{172K}{\pmnum{31.84}{1.01}}{\pmnum{72.04}{1.02}}{2.3$\times$}
% \benchrow{12.50}{21K}{4}{2.0}{258K}{\pmnum{59.66}{2.38}}{\pmnum{107.43}{0.91}}{1.80$\times$}
% \benchrow{12.50}{21K}{4}{4.0}{430K}{\pmnum{119.26}{4.42}}{\pmnum{179.61}{1.51}}{1.51$\times$}

% \benchrow{12.50}{21K}{8}{0.0}{172K}{\pmnum{11.25}{0.74}}{\pmnum{71.83}{1.00}}{\textbf{6.4$\times$}}
% \benchrow{12.50}{21K}{8}{0.2}{215K}{\pmnum{23.77}{0.80}}{\pmnum{89.97}{1.81}}{3.8$\times$}
% \benchrow{12.50}{21K}{8}{0.5}{258K}{\pmnum{36.69}{0.98}}{\pmnum{107.31}{0.69}}{2.9$\times$}
% \benchrow{12.50}{21K}{8}{1.0}{344K}{\pmnum{65.71}{2.13}}{\pmnum{143.58}{1.67}}{2.2$\times$}
% \benchrow{12.50}{21K}{8}{2.0}{516K}{\pmnum{123.25}{5.59}}{\pmnum{214.59}{1.27}}{1.74$\times$}
% \benchrow{12.50}{21K}{8}{4.0}{860K}{\pmnum{249.84}{10.31}}{\pmnum{361.04}{3.19}}{1.45$\times$}

\bottomrule
\end{tabular}
\end{table*}


==> tables/short_qc_old.tex <==
% =========================
% Table 1 (Sparse Forcing merged into chunk-wise block)
% =========================
\begin{table*}[t]
  \centering
  \caption{Comparison with relevant baselines. We compare Sparse Forcing with representative open-source video generation models of comparable scale and resolution. $^{\blacklozenge}$ indicates with awareness pretraining. $^{\diamond}$ indicates without pretraining.}
  \label{tab:short_video_comparison_baselines}

  \footnotesize
  \setlength{\tabcolsep}{3.5pt}
  \renewcommand{\arraystretch}{1.10}

  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}X c c c c c c c}
    \toprule
    \multirow{2}{*}{Model} &
    \multirow{2}{*}{\#Params} &
    \multirow{2}{*}{Resolution} &
    \multirow{2}{*}{\makecell[c]{Throughput\\(FPS) $\uparrow$}} &
    \multirow{2}{*}{\makecell[c]{Latency\\(s) $\downarrow$}} &
    \multicolumn{3}{c}{Evaluation scores $\uparrow$} \\
    \cmidrule(lr){6-8}
    & & & & & Total & Quality & Semantic \\
    \midrule

    \multicolumn{8}{l}{\textbf{Diffusion models}} \\
    LTX-Video\cite{hacohen2024ltx} & 1.9B & $768{\times}512$ & 8.98 & 13.5 & 80.00 & 82.30 & 70.79 \\
    Wan2.1\cite{wan2025wan}    & 1.3B & $832{\times}480$ & 0.78 & 103  & 84.26 & 85.30 & 80.09 \\
    \midrule

    \multicolumn{8}{l}{\textbf{Chunk-wise autoregressive models}} \\
    SkyReels-V2\cite{chen2025skyreels} & 1.3B & $960{\times}540$ & 0.49 & 112 & 82.67 & 84.70 & 74.53 \\
    MAGI-1\cite{teng2025magi}      & 4.5B & $832{\times}480$ & 0.19 & 282 & 79.18 & 82.04 & 67.74 \\
    % CausVid [100]$^{*}$ & 1.3B & $832{\times}480$ & 17.0 & 0.69 & 81.20 & 84.05 & 69.80 \\
    CausVid\cite{yin2025slow} & 1.3B & $896{\times}512$ & - & - & 82.69 & 83.73 & 78.49 \\

    % Self Forcing is a baseline: remove "Ours"
    % Self Forcing (chunk-wise) &
    % 1.3B & \makecell[c]{$832{\times}512$\\(96 frames)} & 17.0 & 0.69 &
    % \textcolor{BestTxt}{\textbf{84.31}} &
    % \textcolor{BestTxt}{\textbf{85.07}} &
    % \textcolor{BestTxt}{\textbf{81.28}} \\

    % ---- merged Sparse Forcing (ours) lines: 5s-length video, DMD checkpoint ----
    Self Forcing\cite{huang2025self} \texttt{L21} &
    1.3B & \makecell[c]{$896{\times}512$} & -- & -- &
    83.88 & 84.60 & 81.01 \\

    \rowcolor{SparseRow}
    Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344}^{\diamond} &
    1.3B & \makecell[c]{$896{\times}512$} & -- & -- &
    83.99 & 84.65 & 81.36 \\

    \rowcolor{SparseRow}
    Sparse Forcing \texttt{BSA0p25\_S3M3L6\_344}^{\blacklozenge} &
    1.3B & \makecell[c]{$896{\times}512$} & -- & -- &
    \textcolor{BestTxt}{\textbf{84.14}} &
    \textcolor{BestTxt}{\textbf{84.84}} &
    \textcolor{BestTxt}{\textbf{81.39}} \\

    \rowcolor{SparseRow}
    Sparse Forcing \texttt{BSA0p25\_S3M3L6\_188}^{\diamond} &
    1.3B & \makecell[c]{$896{\times}512$} & -- & -- & 83.91
     & 84.58 & 81.24 \\

    \rowcolor{SparseRow}
    Sparse Forcing \texttt{BSA0p25\_S3M3L6\_188}^{\blacklozenge} &
    1.3B & \makecell[c]{$896{\times}512$} & -- & -- &
    \textcolor{BestTxt}{\textbf{}} &
    \textcolor{BestTxt}{\textbf{}} &
    \textcolor{BestTxt}{\textbf{}} \\

    % \midrule
    
    % \multicolumn{8}{l}{\textbf{Autoregressive}$^{\dagger}$} \\
    % NOVA [13]         & 0.6B & $768{\times}480$ & 0.88 & 4.1 & 80.12 & 80.39 & 79.05 \\
    % Pyramid Flow [33] & 2B   & $640{\times}384$ & 6.7  & 2.5 & 81.72 & 84.74 & 69.62 \\

    % % Self Forcing baseline: remove "Ours"
    % Self Forcing (frame-wise) &
    % 1.3B & \makecell[c]{$832{\times}512$\\(84 frames)} & 8.9 & 0.45 &
    % 84.26 & 85.25 & 80.30 \\
    \bottomrule
  \end{tabularx}

  \vspace{2pt}
  % {\scriptsize
  % $^{*}$ We compare with the official implementation of CausVid that uses the same base model (Wan-1.3B). \\
  % $^{\dagger}$ The distinction of AR/non-AR applies to the temporal dimension. \\
  % $^{\ddagger}$ 5s-length video results using a DMD checkpoint; FPS/latency are not reported (marked as “--”). \\
  % \textit{Note:} Scores in the DMD block are reported on a $[0,1]$ scale in logs and are multiplied by $100$ here for consistency with the main table.
  % }
\end{table*}


==> tables/theoretical_KV.tex <==

\begin{table}[t]
\centering
\caption{Theoretical KV-cache memory and compute complexity for autoregressive video generation.
Let $h,w$ be spatial tokens per frame, $t$ the number of generated frames, $T$ the total temporal context,
and $S$ the number of denoising (sampling) steps per frame. We report KV memory footprint and the dominant
attention compute (per denoising step and total over $S$ steps). $C_2$ is the sliding-window length in
Self-Forcing; $(C_0+C_1)$ is the effective retained context in Sparse-Forcing (e.g., sink/global + persistent).}
\label{tab:complexity}
\vspace{1mm}
\begin{tabular}{lccc}
\toprule
Method & KV memory & Attention compute / step & Total attention compute ($\times S$) \\
\midrule
Full Attention
& $hwT$
& $hwt \cdot hwT$
& $S \cdot \big(hwt \cdot hwT\big)$ \\

Self Forcing (Sliding Window)
& $C_2 hwt$
& $hwt \cdot (C_2 hwt)$
& $S \cdot \big(hwt \cdot (C_2 hwt)\big)$ \\

Sparse Forcing
& $(C_0+C_1) hwt$
& $hwt \cdot \big((C_0+C_1) hwt\big)$
& $S \cdot \Big(hwt \cdot \big((C_0+C_1) hwt\big)\Big)$ \\
\bottomrule
\end{tabular}
\end{table}
